eLinda: Explorer for Linked Data

To realize the premise of the Semantic Web towards knowledgeable machines, one might often integrate an application with emerging RDF graphs. Nevertheless, capturing the content of a rich and open RDF graph by existing tools requires both time and expertise. We demonstrate eLinda - an explorer for Linked Data. The challenge addressed by eLinda is that of understanding the rich content of a given RDF graph. The core functionality is an exploration path, where each step produces a bar chart (histogram) that visualizes the distribution of classes in a set of nodes (URIs). In turn, each bar represents a set of nodes that can be further expanded through the bar chart in the path. We allow three types of explorations: subclass distribution, property distribution, and object distribution for a property of choice.

==> ls <==
\begin{figure}
	\centering
	%\includegraphics[width=\columnwidth,trim={2cm 2cm 10cm 4cm},clip]{elindaSystem}
        \input{arch.pspdftex}
	\caption{Basic system architecture}
	\label{architecture}
\end{figure}


\section{System Architecture}


The architecture design of \elinda is driven primarily by the
challenge of responsiveness---expansions should happen instantly,
preferably in tens to hundreds of milliseconds.  Specifically, each
exploration step is realized by one or more SPARQL queries, and those
should be performant. However, the queries that are generated by
\elinda are of a restricted form, and we take advantage of this fact.
Moreover, some heavy queries are submitted repeatedly, and we can
enhance the performance using caching and views. Therefore, \elinda
includes several performance enhancements, in both frontend and
backend.

Figure~\ref{architecture} depicts the system architecture of
\elinda. Each SPARQL query is being sent to a \e{reverse proxy}, which
is an Nginx\footnote{\url{https://nginx.org/}} server.  The reverse
proxy handles load balancing and caching policies. Unless cached,
queries are routed to a
Virtuoso\footnote{\url{https://virtuoso.openlinksw.com/}} endpoint.
As we explain next, we use two versions of the Virtuoso endpoint. The
answer is then returned to the client and cached.  Our cache is a
dynamic file based key-value store, implementing an LRU policy. The
key of each entry is the query, and the value is the result.  In
addition to caching, we deploy two techniques for enhancing latency.
\begin{itemize}
\item \textbf{Incremental evaluation.}\,\,  ???
\item \textbf{Materialized views.}\,\,  ???
\end{itemize}

Figure~\ref{queryByStore} shows the performance of the slowest and
most commonly used queries by \elinda. These queries construct the bar
charts of the outgoing and incoming property expasnsion in first
level. The runtime of these queries on the Virtuoso SPARQL endpoint is
454 and 124 seconds for the outgoing and incoming bar charts,
respectively. Extracting the results directly from the cache takes
around 80 milliseconds for both queries. On the Virtuoso SQL endpoint
that uses the materialized views, the queries take 1.5 and 1.2
seconds, respectively.

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{QueryByStore.pdf}
	\caption{Running times of leve-zero property expansions over
          different store configrations}
	\label{queryByStore}
\end{figure}


\eat{

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth,trim={1cm 3cm 1cm 3cm},clip]{QueryByStore}
	\caption{Level zero properties expansion queries runtime over different store configrations}
	\label{queryByStore}
\end{figure}


One of the key requirements of \elinda is responsiveness, which means
reacting quickly to the exploration commands of the user. For a user
interface to be responsiveness, each operation should return a
response in less than half a second. In the case of \elinda{}, each
exploration step include at least one SPARQL query. Unfortunately, the
runtime of some of these SPARQL queries is up to several
minutes. Therefore, to achieve a responsive system we offer several
performance enhancements both in the front end and the back end, as a
dedicated optimized endpoint.



Figure~\ref{architecture} presents our optimized system
architecture. Each SPARQL query to our endpoint is sent first to a
Reverse Proxy called Nginx~\ref{}. The reverse proxy is in charge on
security, load balancing and caching scheme. If this is the first
SPARQL query of this type, route it to the SPARQL endpoint. The SPARQL
endpoint returns the reply to the Reverse Proxy, which in turn route
it to the client and save it in our second component, the cache. Our
cache is a dynamic file based key-value store. The key of each entry
is the query, and the value is the result. We use an LRU caching
scheme and each entry expires after a day. If the same query will be
sent to our endpoint in the next day, the result will be returned
directly from the cache.


Unfortuonately, most SPARQL endpoints return a timeout after a few
seconds and the results of these queries will never be returned and
cached. To solve this problem we offer two solutions. The first is
using an iterative query that builds the graph in steps. In this case
the user first receive initial results, and the longer he waits the
more accurate the results become. The second is constructing an
\elinda{} specialized endpoint as shown in
Figure~\ref{architecture}. Our endpoint use a Virtuoso server that
mirrors the supported knowledge bases. In our endpoint we translate
the property expansion SPARQL queries to SQL and use two specialized
indices, for the ingoing and outgoing. These indices prevents
recomputing the same intermediate results of the property expansion
each time and can be used for all the property expansion
queries. Figure~\ref{queryByStore} shows that computing the queries on
our \elinda{} endpoint reduce the initial property expansion queries
to 1.5 and 1.2 seconds for outgoing and ingoing respectively.  }


==> related.tex <==
\section{Related Work}
% effective visualization = overview + details
% many LD browsers. They are good for understanding the data, the details. Start with a resource then expand. Problems: overview. Many do not show overview at all, some show but limited (survey). Another problem: should know a starting point. Deligiannidis shows improvement but still. 




==> system.tex <==
\section{The System}
% start here with explaining the context diagram
In this section we describe the key components of \elinda{}'s user interface. However, before we do that, we briefly discuss the context in which \elinda{} operates emphasizing its interactions with external systems.

\subsection{Overall Architecture}
\begin{figure}
	\centering
	\includegraphics[height=3in, width=5in]{architecture}
	\caption{eLinda's Context Diagram}
	\label{context}
\end{figure}
\elinda{}'s Context Diagram is presented in Figure \ref{context}.
\elinda{} is a single-page web application that operates within a standard web browser. When a user points the browser to \elinda{}'s URL, an HTML5 page and utility \js{} libraries are fetched from an HTTP server (\textit{Setup} area in the figure).

The HTTP server does not provide \elinda{} with any data to present, neither in the initial setup nor during the subsequent operation of the tool. The data comes from a different source -- a \sparql{} endpoint that \elinda{} is configured to work with.

During its operation (\textit{Exploration} area in the figure), \elinda{} sends dozens of \sparql{} queries to the endpoint, and visually presents the results\footnote{For that purpose, \elinda{} uses the \textsc{AMCHARTS} \js{} library, https://www.amcharts.com.}. To properly handle the large amount of \sparql{} queries sent to the server, a query management library that we have developed mediates between \elinda{} and the \sparql{} endpoint. The library takes care of aspects such as query timeout, failed queries, query resubmission, and query reuse.

\subsection{User Interface}
A \linkeddataset{} is represented in \rdf{} triplet format, where each triplet consists of a \textit{subject}, a \textit{property} (or predicate), and an \textit{object}. \elinda{} provides a Setting Area where the location of a \linkeddataset{} (\sparql{} endpoint) is set by the user. When a new location is set, initial \sparql{} queries are sent to the endpoint to retrieve general statistics such as the total number of triplets, and the number of \textit{classes} that the \linkeddataset{} defines.

For any \linkeddataset{}, classes play an important role since they are part of its \textit{ontology}. Classes themselves are defined using \rdf{} triplets, where typically, the property \textit{rdfs:subClassOf} is used to define an inheritance relationship between classes. An exploration of a \linkeddataset{} using \elinda{} is based on that class hierarchy structure.

\subsubsection{Exploration Pane and Subclasses View}
An Exploration Pane is a multi-tabbed frame supporting the exploration of a single class. \elinda{}'s User Experience (UX) is based on opening more and more Exploration Panes that are laid one beneath the other, where unused Panes can also be closed. Within an Exploration Pane, the first tab that is visible to the user is a Subclass View -- a column chart showing the direct subclasses of the class under exploration.

The user is initially presented with a single Exploration Pane for the root of all classes. In \dbpedia{} for example, that root is the class \textit{owl:Thing}. The Subclass View within that Pane therefore shows all the classes in the first hierarchy level. Each class has its own column, where a class with more instances, i.e., having more \textit{subjects} of its type, is presented earlier in the diagram. Hovering a class' column reveals additional information such as the number of instances and direct subclasses, and a short textual description.

Based on that info, the user can further explore a class of interest by simply clicking it. Additional \sparql{} queries are sent to the endpoint, and another Exploration Pane is created below the previous one, with a similar Subclass View that is now showing the subclasses of the selected class. Similarly, the user may continue the exploration down the class hierarchy.

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.8\textwidth]{MusicalWorkSubClasses}
	%\includegraphics{architecture}
	\caption{Exploration Pane for \dbpedia{}'s class MusicalWork, opened with the Subclasses View.}
	\label{MusicalWorkSubClasses}
\end{figure*}

In Figure \ref{MusicalWorkSubClasses}, we see a third level Exploration Pane showing the subclasses of \dbpedia{}'s MusicalWork class. In the upper-left corner of the Pane we see a Breadcrumb showing a navigation path down to the current class. On top of it we can see how many instances and subclasses the class MusicalWork has. Note that two classes appear with an empty column since they barely have instances (one instance per each). A popup is shown for the first Album subclass revealing that the class has no subclasses, and 132,945 instances.

\subsubsection{Properties View}
Another tab in the Exploration Pane is the Properties View that presents the properties of the class under exploration. We distinguish between \textit{outgoing} properties, where the class' instances act as a subject, and \textit{ingoing} properties, where they act as an object. The Property View consists of two separate diagrams for each type of property.

A column chart is used also here, where each column refers to a specific property found among instances of the class. The properties are sorted based on their \textit{coverage}. A 100\% coverage means that all class' instances share that property. Another calculated metric, \textit{average per instance}, refers to the average occurrence of the property among those instances that share it. For example, in a case that half of the instances share a property and the property occurs multiple times per instance, \textit{coverage} will be 50\% and \textit{average per instance} will be higher than 1.

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.8\textwidth]{MusicalWorkProperties}
	%\includegraphics{architecture}
	\caption{Exploration Pane for \dbpedia{}'s class MusicalWork, opened with the Properties View.}
	\label{MusicalWorkProperties}
\end{figure*}

Figure \ref{MusicalWorkProperties} shows the Property View with outgoing properties, for the \dbpedia{} class MusicalWork whose subclasses were shown earlier. The preparation of the Property View involves querying for all properties attached to any class instance and then sorting them by coverage. Therefore, the result set may include properties with very low coverage that may be of no interest for the user. The coverage threshold in the upper-right corner of the Property View causes the view to present only those properties whose coverage is higher than a supplied user value. In the figure, we see 42 properties with coverage higher than 20\%, the default threshold. 2,230 properties with a lower coverage are excluded from the view.

\subsubsection{Instances View}
The views shown so far allow the user to explore the \linkeddataset{} down the class hierarchy and identify significant classes and properties. However, the user, after finding classes and properties of interest, may wish to explore the actual \textit{data}, and even to retrieve part of the dataset. This gap is filled by the Instances View.

The use of the Instances View follows that of the Properties View. The user should first select properties of interest, as shown in Figure \ref{MusicalWorkProperties}, where two properties of the MusicalWork class where chosen, \textit{name} and \textit{artist} (marked with red). Moving to the Instances View will show the user sample data in a tabular format that corresponds to the selected properties. The user can further filter the data based on one or more columns, and eventually get a \sparql{} query matching the data.

The query shown in Listing \ref{MusicAlbumBobDylan} was generated by \elinda{} after filtering the artist field for "Bob Dylan". The query returns a tabular result set with 185 rows, corresponding to Music Albums whose artist is Bob Dylan.

% Having problems with installing thw listings package..
%\begin{lstlisting}[frame=single]
%SELECT distinct ?subject AS ?mainSubject   ?o1 AS ?name ?o2 AS %?artist   WHERE {?subject a %<http://dbpedia.org/ontology/MusicalWork>.  ?subject %<http://dbpedia.org/property/name> ?o1 .  ?subject %<http://dbpedia.org/ontology/artist> ?o2 .FILTER regex(?o2, %"Bob_Dylan","i"). }
%\end{lstlisting}

 



